Neural Controlled Differential Equations for Online Prediction Tasks

Neural controlled differential equations (Neural CDEs) are a continuous-time extension of recurrent neural networks (RNNs), achieving state-of-the-art (SOTA) performance at modelling functions of irregular time series. In order to interpret discrete data in continuous time, current implementations rely on non-causal interpolations of the data. This is fine when the whole time series is observed in advance, but means that Neural CDEs are not suitable for use in \textit{online prediction tasks}, where predictions need to be made in real-time: a major use case for recurrent networks. Here, we show how this limitation may be rectified. First, we identify several theoretical conditions that interpolation schemes for Neural CDEs should satisfy, such as boundedness and uniqueness. Second, we use these to motivate the introduction of new schemes that address these conditions, offering in particular measurability (for online prediction), and smoothness (for speed). Third, we empirically benchmark our online Neural CDE model on three continuous monitoring tasks from the MIMIC-IV medical database: we demonstrate improved performance on all tasks against ODE benchmarks, and on two of the three tasks against SOTA non-ODE benchmarks.

==> other/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work? 
    \answerYes{\Cref{sec:discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{\Cref{apx:ethics}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Contained along with the proofs in \Cref{apx:ncdes,apx:theoretical}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Proofs are contained in \Cref{apx:ncdes,apx:theoretical}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Included as a zip file in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Included in \Cref{apx:experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All experiments are run 3 times and the standard deviations can be seen in the results tables.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the `Computing infrastructure' paragraph in \cref{apx:experiments_general}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Tan 2020 for Beijing, Warden 2018 for SpeechCommands, Bagnall 2018 for CharacterTrajectories, Johnson 2021 for MIMIC-IV. All are cited in the body of the paper.}
  \item Did you mention the license of the assets?
    \answerYes{See the Datasets section of \Cref{apx:ethics}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{We did not use any new assets.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Consent is required from MIMIC-IV and details are given in \Cref{apx:ethics}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{This is stated in \Cref{apx:ethics}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> tables/base.tex <==
\begin{table*}
    \centering
    % \cmidrule(lr){3-5}
    % TABULAr
    % \hdash
	\caption{}
    \label{tab:wesad_results}
\end{table*}

==> tables/interpolation_irregular.tex <==
\begin{table*}
    \footnotesize
    \centering
    
    % -------------------------
    % TABLE GOES HERE
    % -------------------------
    
    % ----- HEADER ----------
    \begin{tabular}{cccc}
    \toprule
     &  & \multicolumn{2}{c}{\textbf{Dataset}} \\
    \cmidrule(lr){3-4}

    \textbf{Interpolation} & \textbf{Matching region} & \textbf{Mortality} & \textbf{LOS} \\
    % ----- HEADER ----------
    
    \midrule
     & Natural cubic &  0.859 $\pm$ 0.003 &               14.5 $\pm$ 0.1 \\
        & Linear &   0.91 $\pm$ 0.003 &               36.9 $\pm$ 0.8 \\
    Mortality    & Cubic &  0.909 $\pm$ 0.002 &               26.0 $\pm$ 0.6 \\
        & Quintic &  0.907 $\pm$ 0.015 &               23.8 $\pm$ 0.2 \\
        & Rectilinear &  0.893 $\pm$ 0.001 &               96.3 $\pm$ 0.1 \\
    \hdash
     & Natural cubic &  0.241 $\pm$ 0.005 &                4.0 $\pm$ 0.0 \\
        & Linear &  0.149 $\pm$ 0.037 &                7.8 $\pm$ 0.2 \\
    LOS    & Cubic &  0.138 $\pm$ 0.025 &                4.2 $\pm$ 0.1 \\
        & Quintic &    0.16 $\pm$ 0.02 &                3.8 $\pm$ 0.0 \\
        & Rectilinear &  0.109 $\pm$ 0.002 &               11.9 $\pm$ 1.0 \\
    \bottomrule
    \end{tabular}



    
    % -------------------------
    % TO HERE
    % -------------------------
    
    % \hdash
	\caption{}
    \label{tab:wesad_results}
\end{table*}



==> tables/interpolation_regular.tex <==
\begin{table*}
    \footnotesize
    \centering
    
    % -------------------------
    % TABLE GOES HERE
    % -------------------------
    
    % ----- HEADER ----------
    \begin{tabular}{cccc}
    \toprule
    \textbf{Dataset} & \textbf{Interpolation}  & \textbf{Metric} & \textbf{NFEs per epoch $\times 10^3$} \\
    
    % ----- HEADER ----------
    \midrule
     & Natural cubic &     77.6 $\pm$ 1.7 &                4.5 $\pm$ 0.1 \\
    \multirow{2}{*}{BeijingPM10}                  & Linear &     77.5 $\pm$ 2.4 &                5.7 $\pm$ 0.1 \\
                      & Cubic &     78.5 $\pm$ 1.6 &                4.7 $\pm$ 0.1 \\
                      & Rectilinear &     79.0 $\pm$ 0.7 &               15.7 $\pm$ 0.4 \\
    \hdash
     & Natural cubic &     53.3 $\pm$ 0.3 &                4.6 $\pm$ 0.1 \\
    \multirow{2}{*}{BeijingPM2pt5}                      & Linear &     51.7 $\pm$ 0.8 &                5.4 $\pm$ 0.3 \\
                          & Cubic &     52.5 $\pm$ 0.7 &                4.8 $\pm$ 0.1 \\
                          & Rectilinear &     52.0 $\pm$ 1.3 &               16.3 $\pm$ 0.4 \\
    \hdash
     & Natural cubic &  0.927 $\pm$ 0.001 &               25.5 $\pm$ 4.3 \\
    \multirow{2}{*}{SpeechCommands}                      & Linear &  0.933 $\pm$ 0.007 &               63.5 $\pm$ 5.0 \\
                          & Cubic &  0.925 $\pm$ 0.004 &               41.6 $\pm$ 0.3 \\
                          & Rectilinear &    0.938 $\pm$ nan &              108.3 $\pm$ nan \\
    \hdash
     & Natural cubic &  0.836 $\pm$ 0.061 &                1.0 $\pm$ 0.2 \\
    \multirow{2}{*}{CharacterTrajectories}                      & Linear &  0.976 $\pm$ 0.015 &                2.2 $\pm$ 0.1 \\
                          & Cubic &    0.993 $\pm$ 0.0 &                1.9 $\pm$ 0.0 \\
                          & Rectilinear &  0.986 $\pm$ 0.005 &                7.9 $\pm$ 0.4 \\
    \bottomrule
    
    \end{tabular}


    % -------------------------
    % TO HERE
    % -------------------------
    
    % \hdash
	\caption{Comparison of the performance of different interpolation schemes trained using an adaptive scheme for \textbf{regularly sampled} datasets.}
    \label{tab:interpolation_regular_4x}
\end{table*}


